The Assembly History of M87 Through Radial Variations in Chemical Abundances of its Field Star And Globular Cluster Populations

We present an extensive study of spectroscopically-derived chemical abundances for M87 and its globular cluster (GC) system. Using observations from the Mitchell spectrograph at McDonald, LRIS at Keck, and Hectospec on the MMT, we derive new metallicity gradients from $\sim 2$ to $140$ kpc. We use a novel hierarchical statistical framework to simultaneously separate the GC system into subpopulations while measuring the metallicity gradients of those subpopulations. We create physically-motivated spectral stacks of the GC subpopulations by leveraging the output of this statistical framework to perform the first application of abundance tagging in a massive ETG to better constrain the origins of the GC subpopulations and, thus, the assembly history of M87. We find a metal-poor, $\alpha$-enhanced population of GCs in both in the inner and outer halo unanticipated by current cosmological simulations of galaxy evolution. We use the remarkably flat metallicity gradients we find for both the metal-rich and metal-poor GC subpopulations in the inner halo as tentative evidence that some amount of the metal-poor GCs formed directly in the halo of M87 at high redshift.

==> mrt_of_gc_metallicities.tex <==
\begin{table}
\begin{tabular}{cccccc}
ID & RA & DEC & [Fe/H] & $\sigma$ & Instrument \\
H47487 & 187.73553 & 12.32802 & -1.16 & 0.30 & LRIS \\
H49585 & 187.67674 & 12.32961 & -0.51 & 0.41 & LRIS \\
H49328 & 187.71423 & 12.32992 & -0.78 & 0.24 & LRIS \\
H47487 & 187.59446 & 12.02249 & -0.80 & 0.37 & Hectospec \\
H49585 & 187.52539 & 12.03362 & -0.40 & 0.23 & Hectospec \\
H49328 & 187.91104 & 12.04288 & -1.17 & 0.39 & Hectospec \\
\end{tabular}
\end{table}

